Rigorous estimates for the relegation algorithm

We revisit the relegation algorithm by Deprit et al. (Celest. Mech. Dyn. Astron. 79:157-182, 2001) in the light of the rigorous Nekhoroshev's like theory. This relatively recent algorithm is nowadays widely used for implementing closed form analytic perturbation theories, as it generalises the classical Birkhoff normalisation algorithm. The algorithm, here briefly explained by means of Lie transformations, has been so far introduced and used in a formal way, i.e. without providing any rigorous convergence or asymptotic estimates. The overall aim of this paper is to find such quantitative estimates and to show how the results about stability over exponentially long times can be recovered in a simple and effective way, at least in the non-resonant case.

==> form.tex <==
\catcode`@=11
\expandafter\ifx\csname capitolo\endcsname\relax
      {\message {lettura formati e definizioni
standard}}\else{\endinput}\fi
\magnification \magstep1
\tolerance=1500\frenchspacing
%
% Fonti di caratteri
%
\font\megafnt=cmbx12 scaled \magstep4
\font\chpfnt=cmbx10 scaled \magstep3
\font\capfnt=cmss17 scaled \magstep2
\font\titfnt=cmbx10 scaled \magstep1
\font\pagfnt=cmsl10
\font\parfnt=cmbx10 scaled \magstep1
\font\sprfnt=cmsl10 scaled \magstep1
\font\teofnt=cmssbx10
\font\tenenufnt=cmsl10
\font\nineenufnt=cmsl9
\font\eightenufnt=cmsl8

\font \usualfont=cmr10
\font \titlefont=cmbx10
\font \smallfont=cmr9
\font \smallbold=cmbx9
\font \subsecfont=cmr8
\font \smallitalic=cmti9
\font \runningfont=cmr6

\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sixrm=cmr6

\font\ninei=cmmi9
\font\eighti=cmmi8
\font\sixi=cmmi6
\skewchar\ninei='177 \skewchar\eighti='177
\skewchar\sixi='177

\font\ninesy=cmsy9
\font\eightsy=cmsy8
\font\sixsy=cmsy6
\skewchar\ninesy='60 \skewchar\eightsy='60
\skewchar\sixsy='60

\font\eightss=cmssq8

\font\eightssi=cmssqi8

\font\ninebf=cmbx9
\font\eightbf=cmbx8
\font\sixbf=cmbx6
\font\fivebf=cmbx5

\font\ninett=cmtt9
\font\eighttt=cmtt8

\hyphenchar\tentt=-1 % inhibit hyphenation in typewriter type
\hyphenchar\ninett=-1
\hyphenchar\eighttt=-1

\font\ninesl=cmsl9
\font\eightsl=cmsl8

\font\nineit=cmti9
\font\eightit=cmti8

\font\tenmsb=msbm10
\font\ninemsb=msbm9
\font\eightmsb=msbm8
\font\sevenmsb=msbm7
\font\sixmsb=msbm6
\font\fivemsb=msbm5
\newfam\msbfam

\font\tenmat=cmss10
\font\ninemat=cmss9
\font\eightmat=cmss8
\font\sevenmat=cmss7
\font\sixmat=cmss6
\font\fivemat=cmss5
\newfam\matfam

\font\tengrk=grxu1000
\font\ninegrk=grxu0900
\font\eightgrk=grxu0800
\font\sevengrk=grxu0700
\font\sixgrk=grxu0600
\font\fivegrk=grxu0500
\newfam\grkfam

\font\tengrm=gsmn1000
\font\ninegrm=gsmn0900
\font\eightgrm=gsmn0800
\font\sevengrm=gsmn0700
\font\sixgrm=gsmn0600
\font\fivegrm=gsmn0500
\newfam\grmfam

\font\tencyr=wncyr10
\font\sevencyr=wncyr7
\font\fivecyr=wncyr5
\newfam\cyrfam
\textfont\cyrfam=\tencyr
\scriptfont\cyrfam=\sevencyr
\scriptscriptfont\cyrfam=\fivecyr
\def\cyr#1{{\fam\cyrfam\relax#1}}
\def\bcyr{{\cyr B}}

\def\msb{\fam\msbfam\tenmsb} \textfont\msbfam=\tenmsb
     \scriptfont\msbfam=\sevenmsb \scriptscriptfont\msbfam=\fivemsb
  \def\mat{\fam\matfam\tenmat} \textfont\matfam=\tenmat
     \scriptfont\matfam=\sevenmat \scriptscriptfont\matfam=\fivemat
  \def\grk{\fam\grkfam\tengrk} \textfont\grkfam=\tengrk
     \scriptfont\grkfam=\sevengrk \scriptscriptfont\grkfam=\fivegrk
  \def\grm{\fam\grmfam\tengrm} \textfont\grmfam=\tengrm
     \scriptfont\grmfam=\sevengrm \scriptscriptfont\grmfam=\fivegrm

\newskip\ttglue
%
% Definizione formato della pagina
%
\newdimen\pagewidth \newdimen\pageheight
\newdimen\ruleht
\hsize=31.6pc  \vsize=44.5pc  \maxdepth=2.2pt
\parindent=19pt
%\hsize=10.5cm  \vsize=15.5cm  \maxdepth=2.2pt
\parindent=19pt
\hfuzz=2pt
\pagewidth=\hsize \pageheight=\vsize \ruleht=.5pt
\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt
\belowdisplayshortskip=4pt plus 3pt
\def\blank{\vskip 12pt}
\def\blankii{\blank\blank}
\def\blankm{\vskip 6pt}
\def\blankq{\vskip 3pt}
%
% Definizione del corpo dei caratteri e dei formati correnti
%
\def\tenpoint{\def\rm{\fam0\tenrm}%
  \def\enufnt{\tenenufnt}%
  \textfont0=\tenrm \scriptfont0=\sevenrm
\scriptscriptfont0=\fiverm
  \textfont1=\teni \scriptfont1=\seveni
\scriptscriptfont1=\fivei
  \textfont2=\tensy \scriptfont2=\sevensy
\scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex
\scriptscriptfont3=\tenex
  \def\it{\fam\itfam\tenit}%
  \textfont\itfam=\tenit
  \def\sl{\fam\slfam\tensl}%
  \textfont\slfam=\tensl
  \def\bf{\fam\bffam\tenbf}%
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\tentt}%
  \textfont\ttfam=\tentt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=12pt
  \let\sc=\eightrm
  \let\big=\tenbig
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \normalbaselines\rm}

\def\ninepoint{\def\rm{\fam0\ninerm}%
  \def\enufnt{\nineenufnt}%
  \textfont0=\ninerm \scriptfont0=\sixrm
\scriptscriptfont0=\fiverm
  \textfont1=\ninei \scriptfont1=\sixi
\scriptscriptfont1=\fivei
  \textfont2=\ninesy \scriptfont2=\sixsy
\scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex
\scriptscriptfont3=\tenex
  \def\it{\fam\itfam\nineit}%
  \textfont\itfam=\nineit
  \def\sl{\fam\slfam\ninesl}%
  \textfont\slfam=\ninesl
  \def\bf{\fam\bffam\ninebf}%
  \textfont\bffam=\ninebf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\ninett}%
  \textfont\ttfam=\ninett
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=11pt
  \let\sc=\sevenrm
  \let\big=\ninebig
  \setbox\strutbox=\hbox{\vrule height8pt depth3pt width\z@}%
  \normalbaselines\rm}

\def\eightpoint{\def\rm{\fam0\eightrm}%
  \def\enufnt{\eightenufnt}%
  \textfont0=\eightrm \scriptfont0=\sixrm
\scriptscriptfont0=\fiverm
  \textfont1=\eighti \scriptfont1=\sixi
\scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy
\scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex
\scriptscriptfont3=\tenex
  \def\it{\fam\itfam\eightit}%
  \textfont\itfam=\eightit
  \def\sl{\fam\slfam\eightsl}%
  \textfont\slfam=\eightsl
  \def\bf{\fam\bffam\eightbf}%
  \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\eighttt}%
  \textfont\ttfam=\eighttt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=9pt
  \let\sc=\sixrm
  \let\big=\eightbig
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width\z@}%
  \normalbaselines\rm}

\def\tenmath{\tenpoint\fam-1 } % use after $ in ninepoint sections
\def\tenbig#1{{\hbox{$\left#1\vbox to8.5pt{}\right.\n@space$}}}
\def\ninebig#1{{\hbox{$\textfont0=\tenrm\textfont2=\tensy
  \left#1\vbox to7.25pt{}\right.\n@space$}}}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}
%
% Definizione macro di allineamento testi
%
\def\corsivo{\enufnt}
\def\destra#1{{\hfill#1}}
\def\footnote#1{\edef\@sf{\spacefactor\the\spacefactor}$^{#1}$\@sf
      \insert\footins\bgroup\ninepoint
      \interlinepenalty100 \let\par=\endgraf
        \leftskip=\z@skip \rightskip=\z@skip
        \splittopskip=10pt plus 1pt minus 1pt \floatingpenalty=20000
        \smallskip\item{$^{#1}$}\bgroup\strut\aftergroup\@foot\let\next}
\skip\footins=12pt plus 2pt minus 4pt % space added when footnote is present
%\count\footins=1000 % footnote magnification factor (1 to 1)
\dimen\footins=30pc % maximum footnotes per page
%
%  Registrazione referenze su file esterno e macro di conteggio
%
\newcount\numbibliogr@fi@
\global\numbibliogr@fi@=1
\newwrite\fileref
\immediate\openout\fileref=\jobname.ref
\immediate\write\fileref{\parindent 30pt}
\def\cita#1#2{\def\us@gett@{\the\numbibliogr@fi@}
\expandafter\xdef\csname:bib_#1\endcsname{\us@gett@}
           \immediate\write\fileref
           {\par\noexpand\item{{[\the\numbibliogr@fi@]\enspace}}}\ignorespaces
           \immediate\write\fileref{{#2}}\ignorespaces
	   \immediate\write\fileausiliario{\string\expandafter\string\edef
	     \string\csname:bib_#1\string\endcsname{\the\numbibliogr@fi@}}
           \global\advance\numbibliogr@fi@ by 1\ignorespaces}
\def\bibref#1{\seindefinito{:bib_#1}
          \immediate\write16{ !!! \string\bibref{#1} non definita !!!}
      \expandafter\xdef\csname:bib_#1\endcsname{??}\fi
      {$^{[\csname:bib_#1\endcsname]}$}}
\def\dbiref#1{\seindefinito{:bib_#1}
          \immediate\write16{ !!! \string\bibref{#1} non definita !!!}
      \expandafter\xdef\csname:bib_#1\endcsname{??}\fi
      {[\csname:bib_#1\endcsname]}}
\def\citaref#1#2{\cita{#1}{#2}\bibref{#1}}
\def\references{\immediate\closeout\fileref
                \par\goodbreak
                \blankii
                \centerline{\parfnt References}
                \nobreak\blank\nobreak
                \input \jobname.ref}
\def\element#1{\par\blank\noindent\hangindent=30pt
               \llap{#1\enspace}\ignorespaces}
\def\capo#1{\immediate\write\fileref
           {\par\hangindent\parindent }\ignorespaces

\immediate\write\fileref{{#1}}\ignorespaces}
\def\acknowledgements{
           \blankii\noindent
           {\parfnt Acknowledgements.\quad\ignorespaces}
           }
%
% Definizione macro di intestazione
%
\def\title#1{\null\blankii\noindent{\titfnt\uppercase{#1}}\blank}
\def\riga{\par\vskip 6pt\noindent}
\def\author#1{\leftskip 1.8cm\smallskip\noindent{#1}\smallskip\leftskip 0pt}
\def\abstract#1{\par\blankii\noindent
          {\ninepoint
            {\bf Abstract. }{\rm #1}}
          \par}
\def\keywords#1{\par\blank\noindent
          {\ninepoint
            {\bf Key words. }{\rm #1}}
          \par}
\def\sunto#1{\par\blankii\noindent
          {\ninepoint
            {\bf Sunto. }{\rm #1}}
          \par}
%
% Definizione macro per la numerazione delle formule, capitoli,
% paragrafi, ecc...
%
%
%  Definizioni generali
\def\seindefinito#1{\expandafter\ifx\csname#1\endcsname\relax}
\newwrite\filesimboli
    \immediate\openout\filesimboli=\jobname.smb
\newwrite\fileausiliario
    \openin1 \jobname.aux

\ifeof1\relax\else\closein1\relax\input\jobname.aux\fi
    \immediate\openout\fileausiliario=\jobname.aux
%
%  Paragrafo
\newdimen\@mpiezz@
\@mpiezz@=\hsize
\newbox\boxp@r@gr@fo
\newcount\nump@r@gr@fo
\global\nump@r@gr@fo=0
\def\section#1#2{
           \global\advance\nump@r@gr@fo by 1
           \xdef\paragrafocorrente{\the\nump@r@gr@fo}
\expandafter\xdef\csname:sec_#1\endcsname{\paragrafocorrente}
           \global\numsottop@r@gr@fo=0
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{#1 --> Section \paragrafocorrente}
\immediate\write\fileausiliario{\string\expandafter\string\edef
\string\csname:sec_#1\string\endcsname{\paragrafocorrente}}
      \write16{Section {\csname:sec_#1\endcsname}.}
           \goodbreak\vskip 24pt plus 6pt\noindent\ignorespaces
              {\setbox\boxp@r@gr@fo=\hbox{\parfnt\noindent\ignorespaces
              {\paragrafocorrente.\quad}}\ignorespaces
             \advance\@mpiezz@ by -\wd\boxp@r@gr@fo
             \box\boxp@r@gr@fo\vtop{\hsize=\@mpiezz@\noindent\parfnt #2}}
           \par\nobreak\vskip 12pt plus 3pt\nobreak
           \noindent\ignorespaces}
\def\secref#1{\seindefinito{:sec_#1}
          \immediate\write16{ !!! \string\secref{#1} non definita !!!}
 \expandafter\xdef\csname:sec_#1\endcsname{??}\fi
      \csname:sec_#1\endcsname
      }
%  Appendice
\newcount\num@ppendice
\global\num@ppendice=64
\def\appendix#1#2{
           \global\advance\num@ppendice by 1
           \xdef\paragrafocorrente{\char\the\num@ppendice}
           \expandafter\xdef\csname:app_#1\endcsname{\paragrafocorrente}
           \global\numsottop@r@gr@fo=0
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{#1 --> Appendice \paragrafocorrente}
      \immediate\write\fileausiliario{\string\expandafter\string\edef
      \string\csname:app_#1\string\endcsname{\paragrafocorrente}}
      \write16{Appendice {\csname:app_#1\endcsname}.}
           \goodbreak\vskip 18pt plus 6pt\noindent\ignorespaces
              {\setbox\boxp@r@gr@fo=\hbox{\parfnt\noindent\ignorespaces
              {\paragrafocorrente.\quad}}\ignorespaces
             \advance\@mpiezz@ by -\wd\boxp@r@gr@fo
             \box\boxp@r@gr@fo\vtop{\hsize=\@mpiezz@\noindent\parfnt #2}}
           \par\nobreak\vskip 9pt plus 3pt\nobreak
           \noindent\ignorespaces}
\def\appref#1{\seindefinito{:app_#1}
          \immediate\write16{ !!! \string\appref{#1} non definita !!!}
          \expandafter\xdef\csname:app_#1\endcsname{??}\fi
      \csname:app_#1\endcsname
      }
%
%  Sottoparagrafo
\newcount\numsottop@r@gr@fo
\global\numsottop@r@gr@fo=0
\def\subsection#1#2{
           \global\advance\numsottop@r@gr@fo by 1
 \xdef\sottoparcorrente{\paragrafocorrente.\the\numsottop@r@gr@fo}
 \expandafter\xdef\csname:sbs_#1\endcsname{\sottoparcorrente}
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{#1 -----> Subsection \sottoparcorrente}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:sbs_#1\string\endcsname{\sottoparcorrente}}
      \write16{Subsection {\csname:sbs_#1\endcsname}.}
           \goodbreak\vskip 9pt plus 2pt\noindent\ignorespaces
 {\setbox\boxp@r@gr@fo=\hbox{\sprfnt\noindent\ignorespaces
              {\sottoparcorrente\quad}}\ignorespaces
             \advance\@mpiezz@ by -\wd\boxp@r@gr@fo
 \box\boxp@r@gr@fo\vtop{\hsize=\@mpiezz@\noindent\sprfnt#2}}
           \par\nobreak\vskip 3pt plus 1pt\nobreak
           \noindent\ignorespaces}
\def\sbsref#1{\seindefinito{:sbs_#1}
          \immediate\write16{ !!! \string\sbsref{#1} non definita !!!}
 \expandafter\xdef\csname:sbs_#1\endcsname{??}\fi
      \csname:sbs_#1\endcsname
      }
%
%  Sottosottoparagrafo
\newcount\numsottosottop@r@gr@fo
\global\numsottosottop@r@gr@fo=0
\def\subsubsection#1#2{
           \global\advance\numsottosottop@r@gr@fo by 1
 \xdef\sottosottoparcorrente{\sottoparcorrente.\the\numsottosottop@r@gr@fo}
 \expandafter\xdef\csname:sss_#1\endcsname{\sottosottoparcorrente}
      \immediate\write\filesimboli{  }
      \immediate\write\filesimboli{-----> Subsubsection \sottosottoparcorrente :
               rif.: #1}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:sss_#1\string\endcsname{\sottosottoparcorrente}}
      \write16{Subsubsection {\csname:sss_#1\endcsname}.}
           \goodbreak\vskip 9pt plus 2pt\noindent\ignorespaces
 {\setbox\boxp@r@gr@fo=\hbox{\sprfnt\noindent\ignorespaces
              {\sottosottoparcorrente\quad}}\ignorespaces
             \advance\@mpiezz@ by -\wd\boxp@r@gr@fo
 \box\boxp@r@gr@fo\vtop{\hsize=\@mpiezz@\noindent\sprfnt#2}}
           \par\nobreak\vskip 3pt plus 1pt\nobreak
           \noindent\ignorespaces}
\def\sssref#1{\seindefinito{:sss_#1}
          \immediate\write16{ !!! \string\sssref{#1} non definita !!!}
 \expandafter\xdef\csname:sss_#1\endcsname{??}\fi
      \csname:sss_#1\endcsname
      }
%
%  Formula
\def\eqalignno#1{\leqalignno{#1}}
\newcount\numformul@
\global\numformul@=0
\def\formula#1{
            \formdef{#1}\ignorespaces
            \leqno{(\csname:frm_#1\endcsname)}
            }
\def\formdef#1{
            \global\advance\numformul@ by 1
            \def\us@gett@{\the\numformul@}
 \expandafter\xdef\csname:frm_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Formula \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:frm_#1\string\endcsname{\us@gett@}}
            }
\def\frmref#1{\seindefinito{:frm_#1}
          \immediate\write16{ !!! \string\frmref{#1} non definita !!!}
 \expandafter\xdef\csname:frm_#1\endcsname{??}\fi
      (\csname:frm_#1\endcsname)}
%
%  Teorema
\newcount\numenunci@to
\global\numenunci@to=0
\def\endclaim{\endgroup
            \par\if F\sp@zi@tur@{\blankq}\gdef\sp@zi@tur@{T}\fi}
\newcount\numteorema
\global\numteorema=0
\def\theorem#1{
            \global\advance\numteorema by 1
            \def\us@gett@{\the\numteorema}
 \expandafter\xdef\csname:thr_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Theorem \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:thr_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Theorem \us@gett@:\quad}\begingroup\enufnt
            \ignorespaces}
\def\theoremnn{
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Theorem:\quad}\begingroup\enufnt
            \ignorespaces}
\def\theoremtx#1#2{
            \global\advance\numteorema by 1
            \def\us@gett@{\the\numteorema}
 \expandafter\xdef\csname:thr_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Theorem \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:thr_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Theorem \us@gett@:
                {\enufnt #2}.\quad}\begingroup\enufnt
            \ignorespaces}
\def\thrref#1{\seindefinito{:thr_#1}
          \immediate\write16{ !!! \string\thrref{#1} non definita !!!}
 \expandafter\xdef\csname:thr_#1\endcsname{??}\fi
      \csname:thr_#1\endcsname}
%
%  Proposizione
\newcount\numproposizione
\global\numproposizione=0
\def\proposition#1{
            \global\advance\numproposizione by 1
            \def\us@gett@{\the\numproposizione}
 \expandafter\xdef\csname:pro_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Proposition \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:pro_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Proposition \us@gett@:\quad}\begingroup\enufnt
            \ignorespaces}
\def\propositionn{
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Proposition:\quad}\begingroup\enufnt
            \ignorespaces}
\def\propositiontx#1#2{
            \global\advance\numproposizione by 1
            \def\us@gett@{\the\numproposizione}
 \expandafter\xdef\csname:pro_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Proposition \us@gett@}
  \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:pro_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Proposition \us@gett@:
               {\enufnt #2}.\quad}\begingroup\enufnt
            \ignorespaces}
\def\proref#1{\seindefinito{:pro_#1}
          \immediate\write16{ !!! \string\proref{#1} non definita !!!}
 \expandafter\xdef\csname:pro_#1\endcsname{??}\fi
      \csname:pro_#1\endcsname}
%
%  Corollario
\newcount\numcorollario
\global\numcorollario=0
\def\corollary#1{
            \global\advance\numcorollario by 1
            \def\us@gett@{\the\numcorollario}
 \expandafter\xdef\csname:cor_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Corollary \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:cor_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Corollary
\us@gett@:\quad}\begingroup\enufnt
            \ignorespaces}
\def\corref#1{\seindefinito{:cor_#1}
          \immediate\write16{ !!! \string\corref{#1} non definita !!!}
 \expandafter\xdef\csname:cor_#1\endcsname{??}\fi
      \csname:cor_#1\endcsname}
%
%  Lemma
\newcount\numlemma
\global\numlemma=0
\def\lemma#1{
            \global\advance\numlemma by 1
            \def\us@gett@{\the\numlemma}
\expandafter\xdef\csname:lem_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Lemma \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:lem_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Lemma \us@gett@:\quad}\begingroup\enufnt
            \ignorespaces}
\def\lemref#1{\seindefinito{:lem_#1}
          \immediate\write16{ !!! \string\lemref{#1} non definita !!!}
 \expandafter\xdef\csname:lem_#1\endcsname{??}\fi
      \csname:lem_#1\endcsname}
%
%  Definizione
\newcount\numdefinizione
\global\numdefinizione=0
\def\definition#1{
            \global\advance\numdefinizione by 1
            \def\us@gett@{\the\numdefinizione}
 \expandafter\xdef\csname:def_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Definition \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:def_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Definition \us@gett@:\quad}\begingroup\enufnt
            \ignorespaces}
\def\definitiontx#1#2{
            \global\advance\numdefinizione by 1
            \def\us@gett@{\the\numdefinizione}
 \expandafter\xdef\csname:def_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1--------> Definition \us@gett@}
 \immediate\write\fileausiliario{\string\expandafter\string\edef
 \string\csname:def_#1\string\endcsname{\us@gett@}}
            \par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
            \noindent{\teofnt Definition \us@gett@:
               {\enufnt #2}.\quad}\begingroup\enufnt
            \ignorespaces}
\def\defref#1{\seindefinito{:def_#1}
          \immediate\write16{ !!! \string\defref{#1} non definita !!!}
 \expandafter\xdef\csname:def_#1\endcsname{??}\fi
      \csname:def_#1\endcsname}
%
%  Dimostrazione
\def\proof{\par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
    \noindent{\teofnt Proof.\quad}\begingroup\ignorespaces}
\def\prooftx#1{\par\if T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
    \noindent{\teofnt Proof #1.\quad}\begingroup\ignorespaces}
\def\endproof{\par\nobreak\quad\nobreak\hfill\nobreak{\enufnt Q.E.D.}
    \endclaim}
%
% Figura
\newcount\numfigur@
\global\numfigur@=0
\newbox\boxfigur@
\newbox\comfigur@
\newdimen\@mpfigur@
\newdimen\m@rfigur@
%\m@rfigur@=.4 cm
\m@rfigur@=2 pc
\@mpfigur@=\hsize
\advance\@mpfigur@ by -2\m@rfigur@
\def\figure#1#2#3{
            \global\advance\numfigur@ by 1
            \def\us@gett@{\the\numfigur@}
            \expandafter\xdef\csname:fig_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1--------> Figure \us@gett@}
      \immediate\write\fileausiliario{\string\expandafter\string\edef
      \string\csname:fig_#1\string\endcsname{\us@gett@}}
      \setbox\boxfigur@\vbox{\centerline{#2}}
      \topinsert
         {\vbox{
               \vskip 1pt
               \box\boxfigur@
               \vskip 4pt}}
      \setbox\comfigur@\vtop{\hsize=\@mpfigur@\parindent 0pt
         {\ninepoint
         {\teofnt Figure \us@gett@.}\enspace{#3}}
      }
      \centerline{\box\comfigur@}
      \endinsert
      \write16{Figure {\csname:fig_#1\endcsname}.}
      }
\def\figcont#1#2{
      \setbox\boxfigur@\vbox{\centerline{#2}}
      \topinsert
         {\vbox{
               \vskip 1pt
               \box\boxfigur@
               \vskip 4pt}}
 \setbox\comfigur@\vtop{\hsize=\@mpfigur@\parindent 0pt
         {\ninepoint
         {\teofnt Figure \figref{#1}.}\enspace{(continued).}}
      }
      \centerline{\box\comfigur@}
      \endinsert
      \write16{Figura (cont) {\csname:fig_#1\endcsname}.}
}
\def\figref#1{\seindefinito{:fig_#1}
          \immediate\write16{ !!! \string\figref{#1} non definita !!!}
 \expandafter\xdef\csname:fig_#1\endcsname{??}\fi
      \csname:fig_#1\endcsname}
% Citazione
\def\citazione{\begingroup
     \everypar{\parshape 1 \m@rfigur@ \@mpfigur@\noindent}}
\def\finecitazione{\endclaim}
%
%  Osservazione/i
\def\remarks{\par\if
T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
    \noindent{\teofnt Remarks.\quad}\ignorespaces}
\def\remark{\par\if
T\sp@zi@tur@{\gdef\sp@zi@tur@{F}}\else{\blankq}\fi
    \noindent{\teofnt Remark.\quad}\ignorespaces}
%
% Tavola
% #1 : numerazione
% #2 : didascalia
% #3 : tabella
\newcount\numt@vol@
\global\numt@vol@=0
\newbox\boxt@vol@
\newbox\comt@vol@
\newdimen\@mpt@vol@
\newdimen\m@rt@vol@
%\m@rt@vol@=.4 cm
\m@rt@vol@=2 pc
\@mpt@vol@=\hsize
\advance\@mpt@vol@ by -2\m@rt@vol@
\def\table#1#2#3{
            \global\advance\numt@vol@ by 1
            \def\us@gett@{\the\numt@vol@}
            \expandafter\xdef\csname:tav_#1\endcsname{\us@gett@}
      \immediate\write\filesimboli{#1 --------> Table \us@gett@}
      \immediate\write\fileausiliario{\string\expandafter\string\edef
      \string\csname:tav_#1\string\endcsname{\us@gett@}}
      \setbox\boxt@vol@\vbox{#3}
      \topinsert
      \setbox\comt@vol@\vtop{\hsize=\@mpt@vol@\parindent 0pt
         {\ninepoint
         {\teofnt Table \us@gett@.}\enspace{#2}}
      }
      \centerline{\box\comt@vol@}
      \vskip 5pt%
      \centerline{\box\boxt@vol@}%
      \endinsert
      \write16{Table {\csname:tav_#1\endcsname}.}
}
\def\tabcont#1#2{
      \setbox\boxt@vol@\vbox{#2}
      \topinsert
      \setbox\comt@vol@\vtop{\hsize=\@mpt@vol@\parindent 0pt
         {\ninepoint
         {\teofnt Table \tabref{#1}.}\enspace{(continued)}}
      }
      \centerline{\box\comt@vol@}
      \vskip 5pt%
      \centerline{\box\boxt@vol@}%
      \endinsert
      \write16{Table {\csname:tav_#1\endcsname}.}
}
\def\tabref#1{\seindefinito{:tav_#1}
          \immediate\write16{ !!! \string\tabref{#1} non definita !!!}
          \expandafter\xdef\csname:tav_#1\endcsname{??}\fi
      \csname:tav_#1\endcsname}
%
% Inibizione spaziatura prima degli enunciati
%
\def\acapo{\par\noindent}
\def\noblank{\gdef\sp@zi@tur@{T}}
%
% Definizioni per l'output
%
\nopagenumbers
\def\testos{\null}
\def\testod{\null}
\headline={\if T\tpage{\gdef\tpage{F}{\hfil}}
 \else{\ifodd\pageno\rightheadline\else\leftheadline\fi}
           \fi}

\gdef\tpage{T}
\def\rightheadline{\hfil{\pagfnt\testod}\hfil{\pagfnt\folio}}
\def\leftheadline{{\pagfnt\folio}\hfil{\pagfnt\testos}\hfil}
\voffset=2\baselineskip
%
\everypar={\gdef\sp@zi@tur@{F}}
\catcode`@=12
%
%   Definizioni simboli d'uso comune
\def\ap{'$\,$}
\def\pmb#1{\setbox0=\hbox{#1}\ignorespaces
    \hbox{\kern-.02em\copy0\kern-\wd0\ignorespaces
    \kern.05em\copy0\kern-\wd0\ignorespaces
    \kern-.02em\raise.02em\box0 }}
\def\gt{>}
\def\lt{<}
\def\rho{\varrho}
\let\flusso=\phi       % questa istruzione DEVE precedere la
                       % ridefinizione di \phi della prossima riga
\def\phi{\varphi}
\def\epsilon{\varepsilon}
\def\vett#1{\pmb{$#1$}}
\def\derpar#1#2{{{{\partial}{#1}}\over{{\partial}{#2}}}}
\def\bderpar#1#2#3{{{{\partial^2}{#1}}\over{{\partial}{#2}\partial{#3}}}}
\def\dderpar#1#2{{{{\partial^2}{#1}}\over{{\partial}{#2}^2}}}
\def\fraz#1#2{{{#1}\over{#2}}}
\def\frac#1#2{{{#1}\over{#2}}}
\def\area{\mathop{\rm area\,}}
\def\grad{\mathop{\rm grad\,}}
\def\cir{\mathord{\rm circ}}
\def\diff{\mathord{\rm d}}
\def\ddiff{\mathord{{\rm d}^2}}
\def\der#1#2{{{{\diff}{#1}}\over{{\diff}{#2}}}}
\def\dder#1#2{{{{\ddiff}{#1}}\over{{\diff}{#2}^2}}}
\def\dpar#1#2{{{{\partial}{#1}}\over{{\partial}{#2}}}}
\def\bdpar#1#2#3{{{{\partial^2}{#1}}\over{{\partial}{#2
}\partial{#3}}}}
\def\ddpar#1#2{{{{\partial^2}{#1}}\over{{\partial}{#2}^
2}}}
\def\reali{\mathinner{\msb R}}
\def\complessi{\mathinner{\msb C}}
\def\toro{\mathinner{\msb T}}
\def\interi{\mathinner{\msb Z}}
\def\naturali{\mathinner{\msb N}}
\def\razionali{\mathinner{\msb Q}}
%\def\poisson#1#2{{\left\{{#1},{#2}\right\}}}
\def\poisson#1#2{\lbrace#1,#2\rbrace}
\def\mod{\mathop{\rm mod}}
\def\dist{\mathop{\rm dist}}
\def\diag{\mathop{\rm diag}}
\def\diam{\mathop{\rm diam}}
\def\dim{\mathop{\rm dim}}
\def\det{\mathop{\rm det}}
\def\Vol{\mathop{\rm Vol}}
\def\codim{\mathop{\rm codim}}
\def\Im{\mathop{\rm Im}}
\def\lie#1{\Lscr_{#1}}
\def\norma#1{\left\|{#1}\right\|}
\def\ordnorma#1{\|{#1}\|}
\def\bignorma#1{\bigl\|{#1}\bigr\|}
\def\Bignorma#1{\Bigl\|{#1}\Bigr\|}
\def\biggnorma#1{\biggl\|{#1}\biggr\|}
%
\def\Ascr{{\cal A}}
\def\Bscr{{\cal B}}
\def\Cscr{{\cal C}}
\def\Dscr{{\cal D}}
\def\Escr{{\cal E}}
\def\Fscr{{\cal F}}
\def\Gscr{{\cal G}}
\def\Hscr{{\cal H}}
\def\Iscr{{\cal I}}
\def\Jscr{{\cal J}}
\def\Kscr{{\cal K}}
\def\Lscr{{\cal L}}
\def\Mscr{{\cal M}}
\def\Nscr{{\cal N}}
\def\Oscr{{\cal O}}
\def\Pscr{{\cal P}}
\def\Qscr{{\cal Q}}
\def\Rscr{{\cal R}}
\def\Sscr{{\cal S}}
\def\Tscr{{\cal T}}
\def\Uscr{{\cal U}}
\def\Vscr{{\cal V}}
\def\Wscr{{\cal W}}
\def\Xscr{{\cal X}}
\def\Yscr{{\cal Y}}
\def\Zscr{{\cal Z}}
%
\def\avet{{\bf a}}
\def\bvet{{\bf b}}
\def\cvet{{\bf c}}
\def\dvet{{\bf d}}
\def\evet{{\bf e}}
\def\fvet{{\bf f}}
\def\gvet{{\bf g}}
\def\hvet{{\bf h}}
\def\ivet{{\bf i}}
\def\jvet{{\bf j}}
\def\kvet{{\bf k}}
\def\lvet{{\bf l}}
\def\mvet{{\bf m}}
\def\nvet{{\bf n}}
\def\ovet{{\bf o}}
\def\pvet{{\bf p}}
\def\qvet{{\bf q}}
\def\rvet{{\bf r}}
\def\svet{{\bf s}}
\def\tvet{{\bf t}}
\def\uvet{{\bf u}}
\def\vvet{{\bf v}}
\def\wvet{{\bf w}}
\def\xvet{{\bf x}}
\def\yvet{{\bf y}}
\def\zvet{{\bf z}}
\def\Avet{{\bf A}}
\def\Bvet{{\bf B}}
\def\Cvet{{\bf C}}
\def\Dvet{{\bf D}}
\def\Evet{{\bf E}}
\def\Fvet{{\bf F}}
\def\Gvet{{\bf G}}
\def\Hvet{{\bf H}}
\def\Ivet{{\bf I}}
\def\Jvet{{\bf J}}
\def\Kvet{{\bf K}}
\def\Lvet{{\bf L}}
\def\Mvet{{\bf M}}
\def\Nvet{{\bf N}}
\def\Ovet{{\bf O}}
\def\Pvet{{\bf P}}
\def\Qvet{{\bf Q}}
\def\Rvet{{\bf R}}
\def\Svet{{\bf S}}
\def\Tvet{{\bf T}}
\def\Uvet{{\bf U}}
\def\Vvet{{\bf V}}
\def\Wvet{{\bf W}}
\def\Xvet{{\bf X}}
\def\Yvet{{\bf Y}}
\def\Zvet{{\bf Z}}
\def\alphavet{{\grk \char'141}}
\def\betavet{{\grk \char'142}}
\def\gammavet{{\grk \char'147}}
\def\deltavet{{\grk \char'144}}
\def\epsilonvet{{\grk \char'145}}
\def\zetavet{{\grk \char'172}}
\def\etavet{{\grk \char'150}}
\def\thetavet{{\grk \char'152}}
\def\iotavet{{\grk \char'151}}
\def\kappavet{{\grk \char'153}}
\def\lambdavet{{\grk \char'154}}
\def\muvet{{\grk \char'155}}
\def\nuvet{{\grk \char'156}}
\def\xivet{{\grk \char'170}}
\def\pivet{{\grk \char'160}}
\def\rhovet{{\grk \char'162}}
\def\sigmavet{{\vec \sigma}}
\def\tauvet{{\grk \char'164}}
\def\upsilonvet{{\grk \char'165}}
\def\phivet{{\grk \char'146}}
\def\chivet{{\grk \char'161}}
\def\psivet{{\grk \char'171}}
\def\omegavet{{\grk \char'167}}
\def\Gammavet{{\grk \char'107}}
\def\Deltavet{{\grk \char'104}}
\def\Thetavet{{\grk \char'112}}
\def\Lambdavet{{\grk \char'114}}
\def\Xivet{{\grk \char'130}}
\def\Pivet{{\grk \char'120}}
\def\Sigmavet{{\grk \char'123}}
\def\Upsilonvet{{\grk \char'125}}
\def\Phivet{{\grk \char'106}}
\def\Chivet{{\grk \char'121}}
\def\Psivet{{\grk \char'131}}
\def\Omegavet{{\grk \char'127}}
%   Simboli per le matrici
\def\Amat{{\mat A}}
\def\Bmat{{\mat B}}
\def\Cmat{{\mat C}}
\def\Dmat{{\mat D}}
\def\Emat{{\mat E}}
\def\Fmat{{\mat F}}
\def\Gmat{{\mat G}}
\def\Hmat{{\mat H}}
\def\Imat{{\mat I}}
\def\Jmat{{\mat J}}
\def\Kmat{{\mat K}}
\def\Lmat{{\mat L}}
\def\Mmat{{\mat M}}
\def\Nmat{{\mat N}}
\def\Omat{{\mat O}}
\def\Pmat{{\mat P}}
\def\Qmat{{\mat Q}}
\def\Rmat{{\mat R}}
\def\Smat{{\mat S}}
\def\Tmat{{\mat T}}
\def\Umat{{\mat U}}
\def\Vmat{{\mat V}}
\def\Wmat{{\mat W}}
\def\Xmat{{\mat X}}
\def\Ymat{{\mat Y}}
\def\Zmat{{\mat Z}}
\def\Gammamat{{\grm \char'107}}
\def\Deltamat{{\grm \char'104}}
\def\Thetamat{{\grm \char'112}}
\def\Lambdamat{{\grm \char'114}}
\def\Ximat{{\grm \char'130}}
\def\Pimat{{\grm \char'120}}
\def\Sigmamat{{\grm \char'123}}
\def\Upsilonmat{{\grm \char'125}}
\def\Phimat{{\grm \char'106}}
\def\Chimat{{\grm \char'121}}
\def\Psimat{{\grm \char'131}}
\def\Omegamat{{\grm \char'127}}
\def\vet#1{\pmb{$#1$}}
\def\csi{\xi}
\def\ilt{\mathrel{\triangleleft}}
%
\def\autore#1{\leftskip 1.8cm\smallskip\noindent{#1}\smallskip\leftskip 0pt}
\tenpoint\rm


